Non-Archimedean GUE corners and Hecke modules

We compute the joint distribution of singular numbers for all principal corners of a $p$-adic Hermitian (resp. alternating) matrix with additive Haar distribution, the non-archimedean analogue of the GUE (resp. aGUE) corners process. In the alternating case we find that it is a Hall-Littlewood process, explaining -- and recovering as a corollary -- results of Fulman-Kaplan. In the Hermitian case we obtain a `marginal distribution' of a formal Hall-Littlewood process with both positive and negative transition `probabilities'. The proofs relate natural random matrix operations to structural results of Hironaka and Hironaka-Sato on modules over the spherical Hecke algebra, yielding other probabilistic statements of independent interest along the way.

==> The_Hermitian_corners_process.tex <==
\section{The Hermitian corners process}\label{sec:herm_corner}
The main result of this section is the following:
\begin{thm}
    \label{thm:herm_corner}
    Fix a positive integer $n$, let $\la \in \Sig_n$, and let $A$ be a random element of $\Her_n(F)$ distributed by the $K$-invariant measure with singular numbers $\la$. Then the singular numbers of its top-left $(n-1) \times (n-1)$ corner $A'$ are given by
    \begin{equation}\label{eq:herm_corner}
        \Pr(\SN(A') = \nu) = \sum_{\kappa \in \Sig_{n-1}} \frac{P_{\la/\kappa}(1;t) P_\kappa(t,\ldots,t^{n-1};t)}{P_\la(1,\ldots,t^{n-1};t)} \cdot \frac{ Q_{\nu/\kappa}(-1;t)P_\nu(t,\ldots,t^{n-1};t)}{P_\kappa(t,\ldots,t^{n-1};t) \Pi_t(-1;t,\ldots,t^{n-1})}
    \end{equation}
    where $t=-q^{-1}$.
\end{thm}

% \RC{the following result should go in an earlier symmetric function background section, once that's created}
% \begin{lemma}
%     \label{thm:stab_poly}
%      Fix $n \in \Z_{\geq 1}$ and positive $k \leq n$, and for any $\mu \in \Sig_k, \nu \in \Sig_{n-k}$ define
%      \begin{equation}
%          \la(D) = (\mu_1+D,\ldots,\mu_k+D,\nu_1,\ldots,\nu_n).
%      \end{equation}
%      Then for any $\bd \in \Z^n$,
%      \begin{multline}
%         P_{\la(D)}(x_1,\ldots,x_n;t)[\bx^{\bd + (D[n])}]  = \\ \left(P_\mu(x_1,\ldots,x_k;t) P_\nu(x_{k+1},\ldots,x_n;t) \Pi_t(x_1^{-1},\ldots,x_k^{-1};x_{k+1},\ldots,x_n)\right)[\bx^\bd]
%      \end{multline}
%     for all sufficiently large $D$. \RC{will need to define bracket notation and bold variables in a background section or else change this}
% \end{lemma}
% \begin{proof}
    


    
%     A more general version of the result in the setting of Macdonald polynomials (with stabilization of coefficients replaced by convergence) is proven in \cite[Theorem 1.5]{van2020limits}. As detailed in \cite[Remark 6]{van2020limits}, the same proof gives the statement here in the Hall-Littlewood case. \RC{this is a bit terse, but writing a full proof would be annoying so we'll leave this unless the referee complains or you want to flesh it out}%, and the same proof gives the stronger stabilization statement the Hall-Littlewood case, as detailed in \cite[Remark 6]{van2020limits}. 
% \end{proof}

\begin{lemma}
    \label{thm:factor_hl}
    Let $\tau_1,\ldots,\tau_{\binom{n}{k}} \in S_n$ be a set of coset representatives for $S_n/(S_k \times S_{n-k})$, let $\mu \in \Sig_k, \nu \in \Sig_{n-k}$, and define
     \begin{equation}
         \la(D) = (\mu_1+D,\ldots,\mu_k+D,\nu_1,\ldots,\nu_n)
     \end{equation}
     for all $D$ large enough such that this is a valid signature. Then 
     \begin{multline}\label{eq:factor_hl}
         P_{\la(D)}(x_1,\ldots,x_n;t) = \\ 
         \sum_{j=1}^{\binom{n}{k}} \tau_j\left( \Pi_t(x_1^{-1},\ldots,x_k^{-1};x_{k+1},\ldots,x_n) x_1^D \cdots x_k^D P_\mu(x_1,\ldots,x_k;t) P_\nu(x_{k+1},\ldots,x_n;t)\right).
     \end{multline}
\end{lemma}
\begin{proof}
    Direct computation:
    \begin{align}
        \begin{split}
            &P_{\la(D)}(x_1,\ldots,x_n;t) = \frac{(1-t)^n}{\prod_i (t;t)_{m_i(\la(D))}}\sum_{\sigma \in S_n} \sigma\left((x_1 \cdots x_k)^D \prod_{i=1}^k x_i^{\mu_i} \prod_{i=k+1}^n x_i^{\nu_{i-k}} \prod_{1 \leq i < j \leq n} \frac{x_i - t x_j}{x_i - x_j}\right) \\ 
            &= \sum_{j=1}^{\binom{n}{k}} \tau_j\left( \Pi_t(x_1^{-1},\ldots,x_k^{-1};x_{k+1},\ldots,x_n) x_1^D \cdots x_k^D \frac{(1-t)^k}{\prod_i (t;t)_{m_i(\mu)}} \sum_{\sigma \in S_k}  \sigma\left(\prod_{i=1}^k x_i^{\mu_i}  \prod_{1 \leq i < j \leq n} \frac{x_i - t x_j}{x_i - x_j} \right)\right. \\ 
            &\left.\times \frac{(1-t)^{n-k}}{\prod_i (t;t)_{m_i(\nu)}} \sum_{\sigma' \in S_{n-k}} \sigma'\left( \prod_{i=k+1}^n x_i^{\nu_{i-k}} \prod_{k+1 \leq i < j \leq n} \frac{x_i - t x_j}{x_i - x_j} \right)\right) \\ 
            &=\text{RHS\eqref{eq:factor_hl}}.
        \end{split}
    \end{align}
\end{proof}
\begin{rmk}
    \Cref{thm:factor_hl} is inspired by, and is morally a special case of, a result \cite[Theorem 1.5]{van2020limits} which was proven in the generality of Macdonald polynomials. We had to reprove it here because we needed an exact equality rather than the slightly weaker limiting statement which was given in that result, making it not literally a special case.%, but this also has the advantage of keeping everything self-contained.
\end{rmk}

% \begin{rmk}
%     A more general result of this type was shown for Macdonald polynomials in \cite[Theorem 1.5]{van2020limits}. In that setting, however, one must take a limit $D \to \infty$ to obtain convergence of coefficients, so the result there does not directly imply \Cref{thm:stab_poly}, which is why we prove it here.
% \end{rmk}


We now give an explicit form of the Pieri case of the Littlewood-Richardson-type coefficients defined earlier.

\begin{prop}
    \label{thm:herm_pieri}
    For any $\nu \in \Sig_n, \mu \in \Sig_{n-1}$ and $D$ large enough so that all $n$-tuples below are valid signatures, 
    \begin{equation}
        c_{(D,0[n-1]),\nu}^{\her,(2D+|\nu|-|\mu|,\mu_1,\ldots,\mu_{n-1})}(t) = \sum_{\kappa \in \Sig_{n-1}} P_{\nu/\kappa}(1;-t)Q_{\mu/\kappa}(-1;-t),
    \end{equation}
    where $c_{\mu,\nu}^{\her,\la}(t)$ is as defined in \eqref{eq:def_herm_lr} \RC{when that's in a def environment, change eqref to ref to def}.
\end{prop}
\begin{proof}
    We have
    \begin{equation}\label{eq:lr_herm_pieri_spec_case}
        P_{(D,0[n-1])}(x_1^2,\ldots,x_1^2;t^2) P_\nu(x_1,\ldots,x_n;-t) = \sum_{\la} c_{(D,0[n-1]),\nu}^{\her,(2D+|\nu|-|\la|,\la)}(t) P_{(2D+|\nu|-|\la|,\la)}(x_1,\ldots,x_n;-t)
    \end{equation}
    by \eqref{eq:def_herm_lr} and homogeneity of Hall-Littlewood polynomials, where the sum is over all $\la  \in \Sig_{n-1}$ for which $(2D+|\nu|-|\la|,\la) \in \Sig_n$. Since Hall-Littlewood polynomials form a basis, it therefore suffices to show
    \begin{multline}\label{eq:lr_suffices}
        P_{(D,0[n-1])}(x_1^2,\ldots,x_1^2;t^2) P_\nu(x_1,\ldots,x_n;-t) \\  = \sum_{\la} \left( \sum_{\kappa \in \Sig_{n-1}} P_{\nu/\kappa}(1;-t)Q_{\la/\kappa}(-1;-t)\right) P_{(2D+|\nu|-|\la|,\la)}(x_1,\ldots,x_n;-t)
    \end{multline} 
    Applying \Cref{thm:factor_hl} to the $D$-dependent polynomial on both sides and letting $\tau_1,\ldots,\tau_n$ be coset representatives of $S_n/(S_1 \times S_{n-1})$, \eqref{eq:lr_suffices} is equivalent to 
    \begin{multline}\label{eq:second_lr_suffices}
            \sum_{j=1}^n \tau_j(\Pi_{t^2}(x_1^{-2};x_2^{2},\ldots,x_n^{2}))P_\nu(x_1,\ldots,x_n;-t) = \\  \sum_{j=1}^n \tau_j\left( \sum_{\la \in \Sig_{n-1}} \left(\sum_{\kappa \in \Sig_{n-1}} P_{\nu/\kappa}(1;-t)Q_{\la/\kappa}(-1;-t)\right) \Pi_{-t}(x_1^{-1};x_2,\ldots,x_n) x_1^{|\nu|-|\la|}P_\la(x_2,\ldots,x_n;-t)\right).
    \end{multline}
    Since $ P_\nu(x_1,\ldots,x_n;-t)$ is symmetric, we may bring it inside $\tau_j$, so to show \eqref{eq:second_lr_suffices} it suffices to show the term-by-term equality 
    \begin{multline}
                \label{eq:cauchy_swap}
        \Pi_{t^2}(x_1^{-2};x_2^{2},\ldots,x_n^{2})P_\nu(x_1,\ldots,x_n;-t) = \\  \sum_{\la \in \Sig_{n-1}} \left(\sum_{\kappa \in \Sig_{n-1}} P_{\nu/\kappa}(1;-t)Q_{\la/\kappa}(-1;-t)\right) \Pi_{-t}(x_1^{-1};x_2,\ldots,x_n) x_1^{|\nu|-|\la|}P_\la(x_2,\ldots,x_n;-t). 
    \end{multline}
    Writing out the Cauchy kernel explicitly and completing the square we see 
    \begin{equation}
        \Pi_{t^2}(x_1^{-2};x_2^{2},\ldots,x_n^{2}) = \Pi_{-t}(x_1^{-1};x_2,\ldots,x_n)\Pi_{-t}(-x_1^{-1};x_2,\ldots,x_n).
    \end{equation}
    By the branching rule,
    \begin{equation}
        P_\nu(x_1,\ldots,x_n;-t) = \sum_{\kappa \in \Sig_{n-1}} P_{\nu/\kappa}(x_1;-t)P_\kappa(x_2,\ldots,x_n;-t).
    \end{equation}
    Hence by the skew Cauchy identity,
    \begin{align}
        \begin{split}
            \text{LHS\eqref{eq:cauchy_swap}} &= \Pi_{-t}(x_1^{-1};x_2,\ldots,x_n) \sum_{\kappa \in \Sig_{n-1}}P_{\nu/\kappa}(x_1;-t) \left( \Pi_{-t}(-x_1^{-1};x_2,\ldots,x_n)P_\kappa(x_2,\ldots,x_n;-t)\right) \\ 
            &= \Pi_{-t}(x_1^{-1};x_2,\ldots,x_n) \sum_{\kappa \in \Sig_{n-1}}P_{\nu/\kappa}(x_1;-t) \sum_{\la \in \Sig_{n-1}} Q_{\la/\kappa}(-x_1^{-1};-t) P_\la(x_2,\ldots,x_n;-t) \\ 
            &= \text{RHS\eqref{eq:cauchy_swap}},
        \end{split}
    \end{align}
    completing the proof.
  %By \Cref{thm:stab_poly}, for any $\bd \in \Z^n$,
    % \begin{multline}
    %     (x_1^{-2D}P_{(D,0[n-1])}(x_1^2,\ldots,x_1^2;t^2) P_\nu(x_1,\ldots,x_n;-t))[\bx^\bd] \\ 
    %     = (\Pi_{t^2}(x_1^{-2};x_2^2,\ldots,x_n^2) P_\nu(x_1,\ldots,x_n;-t))[\bx^\bd]
    % \end{multline}
    % for all $D$ sufficiently large. It is easy to see that the coefficient on the right hand side is $0$ whenever $\bd > \nu$ in the lexicographic order, since 
    % \begin{equation}
    %     P_\nu(x_1,\ldots,x_n;-t) = \bx^\nu + \text{(lower degree terms)}
    % \end{equation}
    % and multiplication by monomials in the series expansion of $\Pi_{t^2}(x_1^{-2};x_2^2,\ldots,x_n^2)$ can only lower the lexicographic degree. Hence by \eqref{eq:lr_herm_pieri_spec_case}, 
    % \begin{equation}\label{eq:0_d>nu}
    %     \sum_{\la \in \Sig_{n-1}} c_{(D,0[n-1]),\nu}^{\her,(2D+|\nu|-|\la|,\la)}(t) x_1^{-2D}P_{(2D+|\nu|-|\la|,\la)}(x_1,\ldots,x_n;-t)[\bx^\bd] = 0
    % \end{equation}
    % whenever $\bd > \nu$, for all $D$ sufficiently large. Furthermore, the \fix{incomplete}
    % % the left hand side of \eqref{eq:0_d>nu} is trivially $0$ whenever $|\bd| \neq |\nu|$ by homogeneity. 
\end{proof}

% \begin{rmk}
%     `Sufficiently large' may be replaced by `$> \max(\mu_1,\nu_1)$' in \Cref{thm:herm_pieri} by being more careful with the proof and that of \Cref{thm:stab_poly}.
% \end{rmk}

\begin{proof}[Proof of \Cref{thm:herm_corner}]
First note that for any $r > \max(\nu_1,\la_1)$, by reducing modulo $\pi^r$ we have
\begin{align}
    \begin{split}
            \Pr(\SN(A') = \nu) &= \Pr(\SN(\diag(1[n-1],\pi^r) A \diag(1[n-1],\pi^r)) = (2r+|\la|-|\nu|,\nu)) \\ 
            &= \bP_{(r,0[n-1]),\la}^{\her,(2r+|\la|-|\nu|,\nu)},
    \end{split}
\end{align}
where the right hand side is as defined in \fix{add ref}. Hence it suffices to compute the right hand side for sufficiently large $r$. By \Cref{thm:her_product_intro} and \Cref{thm:herm_pieri}, 
\begin{multline}
    \bP_{(r,0[n-1]),\la}^{\her,(2r+|\la|-|\nu|,\nu)} = \frac{P_{(2r+|\la|-|\nu|,\nu)}(1,-q^{-1},\ldots,(-q^{-1})^{n-1};-q^{-1})}{P_{(r,0[n-1])}(1,q^{-2},\ldots,(q^{-2})^{n-1};q^{-2}) P_\la(1,-q^{-1},\ldots,(-q^{-1})^{n-1};-q^{-1})} \\ 
    \times \sum_{\kappa \in \Sig_{n-1}} P_{\la/\kappa}(1;-q^{-1})Q_{\nu/\kappa}(-1;-q^{-1}).
\end{multline}
Moving terms, the above is
\begin{equation}\label{eq:wts=1}
        \frac{P_{(2r+|\la|-|\nu|,\nu)}(1,-q^{-1},\ldots,(-q^{-1})^{n-1};-q^{-1})\Pi_{-q^{-1}}(-1;-q^{-1},\ldots,(-q^{-1})^{n-1})}{P_\nu(-q^{-1},\ldots,(-q^{-1})^{n-1};-q^{-1})P_{(r,0[n-1])}(1,q^{-2},\ldots,(q^{-2})^{n-1};q^{-2})} \cdot \text{RHS\eqref{eq:herm_corner}},
\end{equation}
so we must show the prefactor in \eqref{eq:wts=1} is $1$. This is a straightforward computation from the definition of the Cauchy kernel and principal specialization formulas \fix{add ref}.

\end{proof}


